Intelligent Histology for Tumor Neurosurgery

The importance of rapid and accurate histologic analysis of surgical tissue in the operating room has been recognized for over a century. Our standard-of-care intraoperative pathology workflow is based on light microscopy and H\&E histology, which is slow, resource-intensive, and lacks real-time digital imaging capabilities. Here, we present an emerging and innovative method for intraoperative histologic analysis, called Intelligent Histology, that integrates artificial intelligence (AI) with stimulated Raman histology (SRH). SRH is a rapid, label-free, digital imaging method for real-time microscopic tumor tissue analysis. SRH generates high-resolution digital images of surgical specimens within seconds, enabling AI-driven tumor histologic analysis, molecular classification, and tumor infiltration detection. We review the scientific background, clinical translation, and future applications of intelligent histology in tumor neurosurgery. We focus on the major scientific and clinical studies that have demonstrated the transformative potential of intelligent histology across multiple neurosurgical specialties, including neurosurgical oncology, skull base, spine oncology, pediatric tumors, and periperal nerve tumors. Future directions include the development of AI foundation models through multi-institutional datasets, incorporating clinical and radiologic data for multimodal learning, and predicting patient outcomes. Intelligent histology represents a transformative intraoperative workflow that can reinvent real-time tumor analysis for 21st century neurosurgery.

==> NOTES.tex <==


TODO
1) Need to add reference to the timeline stuff
2) Consider adding a map, that includes all the places that have contributed


1. Workflow/Architecture overview
    Imager, two channel images, virtual stain, etc.

2. AI integration


OUTLINE
Intro
Label-free optical imaging
Intro to label-free optical imaging: SRH, third harmonic, OTC, mention confocal and convivo
Fiber-laser intraoperative Stimulated Raman Histology
Deep learning/AI
Neural networks and deep learning
Medical computer vision
Clinical applications
Intraoperative diagnosis
Stereotactic biopsies
Near-real time brain tumor diagnosis
Molecular classification
Molecular marker prediction
5-ala paper
Lymphoma paper
Tumor recurrence versus pseudoprogression
Tumor recurrence paper
Tumor infiltration detection
Tumor infiltration quantification
Tumor margin sampling and resection guidance
Future directions
Optical phenotypes and real-time prognostication
Prediction of MGMT
Generative models for discoverable optical imaging biomarkers
Intraoperative single cell data
Tumor intrinsic neurons
Immune cell quantification
Label-free single cell tumor infiltration
Multimodal AI-guided glioma surgery
Optical-MRI data, eg. co-registration
Summary


Meningioma resection, take from the Neurosurgery paper
Medical cavernous sinus wall resection




==> latex/commands.tex <==

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}
\newcommand{\tsc}[1]{\textsuperscript{#1}}
\newcommand{\tbf}[1]{\textbf{#1}}
\newcommand{\mbf}[1]{\boldsymbol{#1}}
\renewcommand{\emph}[1]{\textit{#1}}
\newcommand{\innerproduct}[2]{\langle #1, #2 \rangle}

\newcommand{\lstm}{\textsc{LSTM}}
\newcommand{\ffw} {\textsc{Ffw}}
\newcommand{\attn}{\textsc{Attn}}
\newcommand{\encoder} {\textsc{Encoder}}
\newcommand{\key} {\textsc{Key}}
\newcommand{\query} {\textsc{Query}}
\newcommand{\ccca}{\textsc{Cca}}
\newcommand{\crossattention}{\textsc{Ca}}
\newcommand{\softmax}{\textrm{softmax}}
\newcommand{\ret}{\textsc{Ret}}
\newcommand{\block}{\textsc{Block}}
\newcommand{\MassiveText} {Massive Text}
\newcommand{\bert}{\textsc{Bert}\xspace}
\newcommand{\model}{\textsc{Model}}
\renewcommand{\encoder}{\textsc{Encoder}}
\newcommand{\knnlm}{k\textrm{NN-LM}}
\newcommand{\knn}{k\textrm{NN}}
\newcommand{\spalm}{\textsc{Spalm}}
\newcommand{\dpr}{\textsc{Dpr}}
\newcommand{\rag}{\textsc{RAG}}
\newcommand{\realm}{\textsc{Realm}}
\newcommand{\fid}{\textsc{FiD}}
\newcommand{\emdr}{\textsc{Emdr}^2}
\newcommand{\retro}{\textsc{Retro}\xspace}
\newcommand{\retroon}{\textsc{Retro[On]}\xspace}
\newcommand{\retrooff}{\textsc{Retro[Off]}\xspace}
\newcommand{\retrofit}{\textsc{Retro}fit\xspace}
\newcommand{\retrofitting}{\textsc{Retro}fitting\xspace}
\newcommand{\lm}{\textsc{Lm}}
\newcommand{\lmc}{\textsc{Lmc}}
\newcommand{\emb}{\textsc{Emb}}
\newcommand{\readout}{\textsc{Read}}
\newcommand{\spli}{\textsc{Split}}
\newcommand{\bpb}{\textrm{bpb}}
\newcommand{\dmodel}{d}
\newcommand{\dffw}{d_{\textrm{ffw}}}
\newcommand{\lcp}{\textrm{LCP}}

\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Jj}{\mathcal{J}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Rr}{\mathcal{R}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Vv}{\mathcal{V}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\Zz}{\mathcal{Z}}



\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\La}{\Lambda}
\newcommand{\si}{\sigma}
\newcommand{\be}{\beta}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\renewcommand{\phi}{\varphi}
\renewcommand{\th}{\theta}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

\newcommand{\hf}{\hat f}
\newcommand{\wtf}{\tilde f}
\newcommand{\tx}{\tilde x}
\newcommand{\ta}{\tilde a}
\newcommand{\tb}{\tilde b}
\newcommand{\ty}{\tilde y}
\newcommand{\tu}{\tilde u}
\newcommand{\tv}{\tilde v}
\newcommand{\tga}{\tilde \ga}
\newcommand{\tf}{\wt{f}}



\newcommand{\ins}[1]{\mathrm{#1}}
\let\Re\relax

\DeclareMathOperator{\Re}{\Rr e}
\DeclareMathOperator{\Imag}{\Ii m}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Sign}{Sign}
\let\Im\relax
\DeclareMathOperator{\Im}{Im}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\cas}{cas}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\GCD}{GCD}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\interop}{int}

\newcommand{\ps}[2]{\langle #1,#2\rangle}

\newcommand{\Calpha}{\mathrm{C}^\al}
\newcommand{\Cbeta}{\mathrm{C}^\be}
\newcommand{\Cal}{\text{C}^\al}
\newcommand{\Ctwo}{\text{C}^{2}}
\newcommand{\Calt}[1]{\text{C}^{#1}}
\newcommand{\Cder}[1]{\mathscr{C}^{#1}}
\newcommand{\lone}{\ell^1}
\newcommand{\ltwo}{\ell^2}
\newcommand{\linf}{\ell^\infty}
\newcommand{\Lone}{\text{\upshape L}^1}
\newcommand{\Ltwo}{\text{\upshape L}^2}
\newcommand{\Linf}{\text{\upshape L}^\infty}
\newcommand{\lzero}{\ell^0}
\newcommand{\lp}{\ell^p}
\newcommand{\Sun}{\text{S}^1}
\newcommand{\foralls}{\forall \,}
\newcommand{\dd}{\ins{d}}
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}



\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\whwh}[1]{\hat{\hat{#1}}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\pd}[2]{ \frac{ \partial #1}{\partial #2} }
\newcommand{\pdd}[2]{ \frac{ \partial^2 #1}{\partial #2^2} }
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\imath}{\mathrm{i}}
\newcommand{\interior}[1]{\ensuremath{\overset{\circ}{#1}}}

\newcommand{\legsymb}[2]{ \genfrac{(}{)}{}{}{#1}{#2} }
\newcommand{\ordin}[2]{ ${#1}^{ \text{#2} }$ }
\newcommand{\dotp}[2]{\langle #1,\,#2\rangle}
\newcommand{\dotps}[2]{\langle #1,\,#2\rangle}
\newcommand{\crossp}[2]{ #1 \hat #2 }
\newcommand{\seg}[2]{\llbracket #1,\,#2 \rrbracket}
\newcommand{\brac}[1]{\left[#1\right]}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\snorm}[1]{\| #1 \|}
\newcommand{\normb}[1]{\Big|\!\Big| #1 \Big |\!\Big|}
\newcommand{\normB}[1]{\left|\!\left| #1 \right|\!\right|}
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator{\Prox}{Prox}
\newcommand{\normT}[1]{\norm{#1}_{\text{T}}}
\newcommand{\normu}[1]{\norm{#1}_{1}}
\newcommand{\normi}[1]{\norm{#1}_{\infty}}
\newcommand{\normd}[1]{\norm{#1}_{2}}
\newcommand{\normz}[1]{\norm{#1}_{0}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert} %
\newcommand{\absb}[1]{\Big| #1 \Big|}

\newcommand{\func}[4]{ {\left\{  \begin{array}{ccc} #1 & \longrightarrow & #2 \\ #3 & \longmapsto & #4 \end{array}  \right.} }
\newcommand{\Id}{\ins{Id}}
\newcommand{\eqdef}{\triangleq}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\pa}[1]{\left( #1 \right)}
\newcommand{\bpa}[1]{\big( #1 \big)}
\newcommand{\choice}[1]{ %
	\left\{ %
		\begin{array}{l} #1 \end{array} %
	\right. }
\newcommand{\set}[1]{ \{ #1 \} }
\newcommand{\condset}[2]{ \left\{ #1 \;;\; #2 \right\} }


\newcommand{\qandq}{ \quad \text{and} \quad }
\newcommand{\qqandqq}{ \qquad \text{and} \qquad }
\newcommand{\qifq}{ \quad \text{if} \quad }
\newcommand{\qqifqq}{ \qquad \text{if} \qquad }
\newcommand{\qwhereq}{ \quad \text{where} \quad }
\newcommand{\qqwhereqq}{ \qquad \text{where} \qquad }
\newcommand{\qwithq}{ \quad \text{with} \quad }
\newcommand{\qqwithqq}{ \qquad \text{with} \qquad }
\newcommand{\qforq}{ \quad \text{for} \quad }
\newcommand{\qqforqq}{ \qquad \text{for} \qquad }
\newcommand{\qqsinceqq}{ \qquad \text{since} \qquad }
\newcommand{\qsinceq}{ \quad \text{since} \quad }
\newcommand{\qarrq}{\quad\Longrightarrow\quad}
\newcommand{\qqarrqq}{\quad\Longrightarrow\quad}
\newcommand{\qiffq}{\quad\Longleftrightarrow\quad}
\newcommand{\qqiffqq}{\qquad\Longleftrightarrow\qquad}
\newcommand{\qsubjq}{ \quad \text{subject to} \quad }
\newcommand{\qqsubjqq}{ \qquad \text{subject to} \qquad }
\newcommand{\qobjq}[1]{\quad \text{#1} \quad}
\newcommand{\qqobjqq}[1]{\quad \text{#1} \quad}





\newlength{\restsubwidth}
\newlength{\restsubheight}
\newlength{\restsubmoreheight}
\setlength{\restsubmoreheight}{4pt}
\newcommand{\rest}[2]{%
        \settowidth{\restsubwidth}{\ensuremath{#2}}
        \settoheight{\restsubheight}{\ensuremath{{}_{#2}}}
        \ensuremath{{#1\hskip 0.5pt}_{\vrule\kern2pt\parbox[b][%
        4pt][b]{\the\restsubwidth}{%
                        \ensuremath{{}_{#2}}}}}
        }


==> latex/extended_data.tex <==

\clearpage
\appendix

\section{Extended Data Figures}
\begin{enumerate}
    \item Expanded Workflow and Prima Architecture
    \item Overview of UM-220K Dataset
    \item LLM annotations and neuroradiology language models
    \item MRI volume tokenization
    \item MRI-report contrastive pre-training
    \item Extended Prima diagnostic performance results
    \item Diverse clinical examples of Prima explainibility
    \item Multi-label analysis of Prima
    \item Extended clinical task and transfer learning results
    \item Subgroup performance and fairness analysis
\end{enumerate}

\section{Supplementary Data}
\subsection{Supplementary Data Figures}
\begin{enumerate}
    \item SQL query for UM-220K search
    \item GPT-3.5 prompt for report summarization with summarized report examples
    \item GPT-4 prompt for report classification
    \item PyTorch-style pseudocode for VQ-VAE with random permutations
    \item PyTorch-style pseudocode for Prima MRI-Report CLIP
\end{enumerate}

\subsection{Supplementary Data Tables}
\begin{enumerate}
    \item Demographic information for UM-220K dataset
    \item Demographic information for prospective testing dataset
    \item Diagnosis-Referral-Priority mapping
    \item Demographic summary of retrospective fairness dataset
    \item Demographic summary of prospective fairness dataset
\end{enumerate}


%%%%%
\clearpage
\renewcommand{\figurename}{Extended Data Figure}
\setcounter{figure}{0}

%%%% EXTENDED DATA FIGURE 1 
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.78]{assets/Ext_Data_Fig1.pdf}
    \caption{\textbf{Expanded Workflow and Prima Architecture}. Caption on next page.}
    \label{exfig:ex_data1}
\end{figure*}

\begin{figure*}[p!]
  \contcaption{\textbf{Expanded Workflow and Prima Architecture} \textbf{a}, Our health system Sectra PACS server was queried for all cranial MRIs. We then filtered these MRIs based on the availability of an associated radiology report and having a minimum of 2 series per study. We then ensured that all metadata was present, resulting in a total of 221,147 UM-220K dataset. \textbf{b}, Overview of the stages of training Prima on UM-220K, which includes volume tokenization, hierarchical ViT training with CLIP objective function, and transfer learning to predict radiologic diagnoses. Radiology report summarization and diagnostic labels are provided by an LLM for reliable, accurate, and scalable vision-language modeling. \textbf{c}, Volume tokenization stage involves dividing each MRI volume into smaller subvolume patches of shape 32x32x4, removing background tokens, and encoding each subvolume using a VQ-VAE encoder. The latent VQ-VAE tokens are then passed forward to the sequence ViT with the concatenated positional encodings. \textbf{d}, The hierarchical ViT is trained using a CLIP objective on frozen volume token features. The sequence ViT is a multimodal transformer that takes as input both the volume tokens and the embedded free-text sequence description. The series registers are passed forward to the study ViT that outputs a single representation for the full MRI study. The paired reports are summarized and passed through a pre-trained neuroradiology model to align the MRI study and the paired report. \textbf{d}, A transfer learning strategy is used where the volume tokenizer, sequence and study transformers are frozen, and an MLP is trained on the learned study features for radiologic and clinical task prediction.}
\end{figure*}


%%%% EXTENDED DATA FIGURE 2
\clearpage
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.78]{assets/Ext_Data_Fig2.pdf}
    \caption{\textbf{Overview of UM-220K Dataset}. Caption on next page.}
    \label{exfig:ex_data2}
\end{figure*}


\begin{figure*}[p!]
\contcaption{\textbf{Overview of UM-220K Dataset}. Descriptive details of the UM-220K dataset are shown here. \textbf{a}, The majority of MRI data is collected from patient's with permanent residence in the state of Michigan. A geospatial map shows the counties with the top 20 imaging centers across the state. The top centers are located in populous regions and regions with higher median income based on census data (www.census.gov). The Upper Peninsula and Northern Michigan are lower resource settings, rural areas, and most susceptible to experiencing longer turnaround times (Fig. 4). \textbf{b}, Average turnaround time through time. We observed a steady year-to-year increase in turnaround time since 2019. This increase correlates with increasing MRI demand and imaging volumes at our health system. \textbf{c}, The distribution of turnaround times. The distribution shows a severe right skew, with a Fisher-Pearson coefficient of skewness of 5.25. The majority of turnaround time measured in patient-days is in the right tail distribution greater than 2 days. These results prompted us to target turnaround time as a metric of algorithmic fairness. \textbf{d}, Distribution of MRI counts through time and divided by month of year. We observed a consistent increase in the number of MRIs/year.  \textbf{e}, Age and sex distribution of the UM-220K. \textbf{f}, Distribution of patients by the number of diagnoses per patient, including patients with no diagnoses. \textbf{g}, Distribution of diagnostic categories and (\textbf{h}) the granular radiology diagnoses for for each category. The aims was to have a broad set of diagnostic categories that spanned the full diagnostic spectra and to include clinically meaningful and actionable diagnostic classes. 
  }
\end{figure*}


%%%% EXTENDED DATA FIGURE 3
\clearpage
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.77]{assets/Ext_Data_Fig3.pdf}
    \caption{\textbf{LLM annotations and neuroradiology language models}. Caption on next page.}
    \label{exfig:ex_data3}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{LLM annotations and neuroradiology language models}. \textbf{a}, Example of an original MRI report with highlighting of the major findings in the MRI study. GPT-3.5-turbo is then prompted in stages to summarized the report to achieve an itemized report summary of positive findings. Additional details regarding prompting are in Supplementary Data Fig. 2 and 3. \textbf{b}, The classification performance of GPT-4 for 5 diagnoses from the different diagnostic categories: structural, adult tumor, cystic lesions, infectious, and vascular ischemic. \textbf{c}, tSNE visualizations of the sequence name encoding after training the sequence name encoder, $E_{sn}$, using a CLIP objective. The model correctly encodes sequence names based on both imaging planes and sequence type. This effectively prompts $ViT_{seq}$ for better MRI sequence feature extraction. \textbf{d}, Line plot shows the average validation perplexity during training of the neuroradiology language model given different percentages of the report data. Neuroradiology language model was trained using next-word prediction and benefits from increased training data, approaching the lower perplexity bound of 1 with 100\% of the MRI reports. \textbf{e}, tSNE plots of the CLIP encoded summarized reports versus full reports. The summarized reports show better label-conditional clustering compared to the full reports. These results demonstrate the challenge of using full reports for CLIP, which contain extraneous or non-informative textual details that can degrade visual representation learning. The center panels are Silhouette plots to quantify cluster quality. The red dotted line is the average Silhouette coefficient. Larger values represent better clustering results.}
\end{figure*}


%%%% EXTENDED DATA FIGURE 4
\clearpage
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.8]{assets/Ext_Data_Fig4.pdf}
    \caption{\textbf{MRI volume tokenization}. Caption on next page.}
    \label{exfig:ex_data4}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{MRI volume tokenization} \textbf{a}, MRI scanners acquire images with specified orientations (e.g. LAS, RAS, etc) and planes (e.g. axial, coronal, sagittal). The MRI tokens will have the same orientation and plane as the source MRI sequence after patching. \textbf{b}, Examples of VQ-VAE reconstructions in different MRI sequences and orientations. \textbf{c}, Because Prima takes as input multiple different orientations and imaging planes, the volume tokenizer should be orientation invariant, meaning the representation of the same anatomic region should not change if imaged in axial versus coronal plane or LAS versus RAS orientation, for example. We used two strategies: random orientation permutations and 3D-CNN encoders. Our VQ-VAE volume tokenizer is encouraged to encode each volume token equivalently across all orientations under a reconstruction loss. Examples of MRI subvolumes are shown in different orientations after permutation. The latent volume tokens with near-equivalent latent encodings are shown in the center panel. with the reconstructions after the decoder on the right.  \textbf{d}, Ablation study over the codebook sizes shows the quantization loss validation curves. Larger codebook sizes led to less overfitting and better reconstructions. \textbf{e}, Reconstruction losses with and without random orientation permutations. Random permutations regularized the VQ-VAE and resulted in higher-quality reconstructions and lower reconstruction losses. \textbf{f}, Examples of reconstructions before and after orientation permutations for different MRI sequences. Reconstructions are perceptually equivalent after forward pass through the VQ-VAE model regardless of orientation or imaging plane. Subtle reconstruction differences can be seen on difference maps.}
\end{figure*}

%%%% EXTENDED DATA FIGURE 5
\clearpage
\begin{figure*}[p!]
    \centering\includegraphics[width=\textwidth]{assets/Ext_Data_Fig5.pdf}
    \caption{\textbf{MRI-report contrastive pretraining}}
    \label{exfig:ex_data5}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{MRI-report contrastive pretraining}. \textbf{a}, Radar performance plot of the model design choices. Prima architecture outperformed other model designs across the majority of diagnostic tasks. Mean prospective AUC (\textbf{b}) and mean ROC curves (\textbf{c}) across model design choices. \textbf{d}, Top 5 image-to-text retrieval accuracy of Prima with and without the patient discrimination loss. We see over a 5x speed-up in training time when using the patient discrimination loss. \textbf{e}, Ablation experiments over the neuroradiology language model. We found that pre-training on radiology reports resulted in more efficient training and that updating the language model during CLIP training was essential for MRI representation learning. \textbf{f}, Mean ROC curves with increased training data. We have not observed an upper bound on performance and the data provides evidence that additional MRI data will continue to improve performance, even at fixed model capacity and compute budget \cite{Kaplan2020-ia}. These results emphasize the importance of health system-scale training and the health system-as-data engine framework.}
\end{figure*}
\clearpage

%%%% EXTENDED DATA FIGURE 6
\begin{figure*}[p!]
    \centering\includegraphics[width=\textwidth]{assets/Ext_Data_Fig6.pdf}
    \caption{\textbf{Extended Prima performance results}}
    \label{exfig:ex_data6}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{Extended Prima performance results} 
    \textbf{a}, Performance in each diagnostic category averaged over the diagnostic tasks. \textbf{b}, Average Top-1 retrieval accuracy on the prospective testing cohort by days of CLIP training. We see a continued, unbounded increase in performance after 50 training days. \textbf{c}, We show the normalized positive rate (NPR) of the top 20 nearest retrospective neighbors for prospective instances on each prediction task. NPR is calculated by $\frac{\text{average positive rate in top 20 nearest retrospective neighbors}}{\text{positive rate in retrospective set}}$. In other words, for any prospective MRI study with a set of positive labels, the NPR indicates how many times as likely the top 20 nearest neighbors are to have same label, compared to the positive rate of the full dataset. For each diagnostic task, we compute NPR averaged across all prospective studies (\textcolor{orange}{orange}) and across positive prospective studies only (\textcolor{blue}{blue}). For example, for Dandy-Walker Malformation (DWM), the prospective positives have an average NPR of 133.91, indicating that the average positive rate of top-20 nearest neighbors of all prospective instances with DWM (4.057 out of 20, around 20\%) is 133.91 times the overall DWM positive rate (335 out of 221147, around 0.151\%). The expected NPR value for randomly distributed examples is 1 (dotted line). The mean NPR for the positive prospective instances (blue bars) exceeds 1 by a large margin. The orange bars are around or less than 1, indicating that the neighbors of positive studies are much more likely to be positive for the same prediction. Therefore, this analysis demonstrates that Prima embeddings tend to group studies with the same diagnoses closer together.}
\end{figure*}
\clearpage

%%%% EXTENDED DATA FIGURE 7
\begin{figure*}[p!]
    \centering\includegraphics[width=\textwidth]{assets/Ext_Data_Fig7.pdf}
    \caption{\textbf{Diverse Clinical Examples of Prima Explainability}. Caption on next page.}
    \label{exfig:ex_data7}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{Diverse Clinical Examples of Prima Explainibility.} We show a diverse selection of patients from our prospective testing cohort with associated LIME importance scores on the volume tokens. The top 5 tokens are color-coded according to the legend above. Prima correctly identifies the pathologic regions in all the clinical scenarios presented above, including pediatric posterior fossa tumors, vascular malformations, ischemic lesions, adult brain tumors, brain cysts, and developmental abnormalities. High LIME score tokens that localize to the pathologic regions demonstrate trustworthy Prima predictions. Red dashed line represented expert annotated pathologic regions.}
\end{figure*}


%%%% EXTENDED DATA FIGURE 8
\clearpage
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.80]{assets/Ext_Data_Fig8.pdf}
    \caption{\textbf{Multi-label analysis of Prima}}
    \label{exfig:ex_data8}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{Multi-label analysis of Prima}
    \textbf{a}, We performed a multi-label classification analysis across all 52 diagnoses. The Prima logit-label matrix above shows the AUC value for each logit-label binary comparison. The diagnoses were ordered using consensus clustering for easier visualization \cite{Monti2003-bo}. The lower left-hand matrix is the correlation matrix of the ground truth labels with the same ordering. Prima learned the label co-occurrence relationships, such as ventriculomegaly often co-occurs with ventricular catheters or brain tumors co-occur with mass effect. It also correctly captures the semantic similarity of diagnoses within differential diagnoses. We observer higher AUC values for related structural pediatric diagnoses, brain tumor diagnoses, and brain injury/trauma. These findings demonstrate that Prima has correctly modeled the multi-label classification problem while learning the semantic relationships between related diagnoses. The same logit-label matrix for the PubMedCLIP model is shown for comparison in the lower right corner. \textbf{b}, Multi-label LIME analysis shows that Prima attends to different pathologic regions of the same MRI sequence depending on the diagnostic prediction. High LIME scores are assigned to tokens within the posterior fossa when the LIME scores are computed for `medulloblastoma' prediction. Conversely, high LIME scores are assigned to the enlarged ventricles when the LIME scores are computed for 'ventriculomegaly' prediction. We see similar patterns investigating the relationship between `brain contusion' and `midline shift' labels, and `brain metastasis' and `vasogenic edema' labels. Prima demonstrates \emph{trusthworthy multi-label classification}.
    }
\end{figure*}
\clearpage


%%%% EXTENDED DATA FIGURE 9
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.77]{assets/Ext_Data_Fig9.pdf}
    \caption{\textbf{Extended clinical task and transfer learning results}. Caption on next page.}
    \label{exfig:ex_data9}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{Extended clinical task and transfer learning results}
    \textbf{a}, Confusion matrices for ordinal metric learning, cross entropy, and binary ordinal losses for MRI prioritization. Cross entropy provided the overall best results. Examples of normal, medium, and high acuity are shown. Most importantly for triage and acuity assessment, misclassification rates were lowest for normal-high discrimination. \textbf{c}, External testing performance on BraTS, Stroke, NYUMets, and UCSFMets datasets. We see true positive rates on par with our prospective testing cohort. \textbf{c}, LIME importance scores extended to the BraTS dataset, identifying volume tokens within the externally annotated tumor regions. An example of both a lower grade diffuse glioma, IDH mutation, and a higher grade glioblastoma, IDH wildtype, MRI are shown. Prima correctly identified the FLAIR hyperintense regions as evidence of tumor infiltration. Contrast enhancing regions of the glioblastoma were most important for high grade glioma classification. \textbf{d}, Quantitative evaluation of LIME volume token selection versus the segmented tumor regions. We show that Top-3 accuracy for Prima selecting volume tokens within the ground truth segmented tumor region was 98.0\%. These results provide external, quantitative evaluation of trustworthy predictions from Prima. \textbf{b}, LIME visualizations for our external acute stroke dataset. An example of an acute middle cerebral artery distribution stroke and a posterior cerebral artery distribution stroke are shown. Prima assigned high LIME score to regions of diffuse restriction on DWI images, indicative of acute ischemia.
    }
\end{figure*}
\clearpage

%%%% EXTENDED DATA FIGURE 10
\begin{figure*}[p!]
    \centering\includegraphics[scale=0.75]{assets/Ext_Data_Fig10.pdf}
    \caption{\textbf{Subgroup performance and fairness analysis}. Caption on next page.}
    \label{exfig:ex_data10}
\end{figure*}

\begin{figure*}[p!]
    \contcaption{\textbf{Subgroup performance and fairness analysis} \textbf{a}, Prima performance for tasks presented in Fig. 4: population, region, and schedule. \textbf{b}, Prima performance and fairness analysis for non-modifiable sensitive attributes: sex, age, and race. Prima showed consistently high performance, on par with the population performance, across all subgroups. Prima demonstrated algorithmic fairness for sex and race; we found a statistically significant difference in TPR disparity for ages between 34-61. These may be related to greater diversity of diagnoses within this subgroup compared to pediatric and older populations. \textbf{c}, Prima performance and fairness analysis for modifiable sensitive attribute: insurance status, MRI manufacturer, and radiologist. Prima did not show statistically significant difference in performance or fairness based on government-sponsored versus private insurers. Importantly, MRI performance was consistent across the three major MRI manufacturers: Seimens, Philips, and GE. P-values are greater than 0.05 with multiple hypothesis correction unless otherwise noted.}}
\end{figure*}

%%%% Supplementary DATA FIGURE 10
\clearpage
% \renewcommand{\figurename}{Supplementary Data Figure}
% \setcounter{figure}{0}

% \begin{figure*}[p!]
%     \centering\includegraphics[scale=0.8]{assets/Supplementary_Figure_1.pdf}
%     \caption{\textbf{TODO}}
%     \label{exfig:supp_data1}
% \end{figure*}

% \begin{figure*}[p!]
%     \centering\includegraphics[scale=0.8]{assets/Supplementary_Figure_2.pdf}
%     \caption{\textbf{TODO}}
%     \label{exfig:supp_data2}
% \end{figure*}



%%%% Algorithm 1 for Permutation Strategy
\begin{figure*}
\vspace{-20pt}
\centering
\small
\begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule}
\begin{algorithm}[H]
\caption{Supplementary Data Figure 4: Random Token Permutation Strategy in PyTorch style}
\label{alg:clip}
\definecolor{codeblue}{rgb}{0.0,0.5,0.0}
\definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
\lstset{
  basicstyle=\fontsize{10pt}{9pt}\lstsansserif\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\color{codeblue},
  keywordstyle=\color{codekw},
}
\begin{lstlisting}[language=python]
# vol_tokenizer: MRI tokenizer function, outputs N dimensional array of F dimensional 3D tokens
# p: function to permute tokens to desired shape
# mb: image minibatches
# V: VQVAE model
# S: set of all image minibatches

def get_randomly_permuted_tokens(mb):
    # Buckets for the 3 unique token shapes (e.g. 4x32x32, 32x4x32, and 32x32x4)
    token_buckets = {(4,32,32): [ ] , (32,4,32): [ ], (32,32,4): [ ] }

    for i in mb:
        # Tokenize each image in the minibatch and find shape of each token
        token_list, token_shape = vol_tokenizer(i)
        # Pass token list to corresponding dictionary pair based on token shape
        token_buckets[token_shape].extend(token_list)
    
    for key in tokens_buckets:
        # Stack all tokens in a given key, value pair
        token_buckets[key] = torch.stack(token_buckets[key])
    
    # Randomly select desired token shape for the minibatch
    selected_shape = random.choice(list(token_buckets.keys()))
    
    return token_buckets[selected_shape].permute(0,*random.shuffle([1,2,3]))

# Get dataset of all tokenized, permuted data
dt = Dataset(get_randomly_permuted_tokens(mb) for mb in Dataset(S))
dl = Dataloader(dt)

# Feed forward each minibatches through VQVAE model
for tokens in dl:
    loss = V(tokens)
    loss.backward()
    optimizer.step()

\end{lstlisting}
\begin{comment}
    % # Permute all tokens to match desired token shape
    % permuted_buckets = {key: p(value, selected_shape) for key, value in token_buckets.items()}

    % # Concatenate all token tensors in minibatch as dataset
    % Return torch.cat([value for value in permuted_buckets.values()], dim=0)

\end{comment}

\end{algorithm}
\end{minipage}
\vspace{-10pt}
\end{figure*}



\begin{figure*}
\vspace{-20pt}
\centering
\small
\begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule}
\begin{algorithm}[H]
\caption{Supplementary Data Figure 5: MRI-Report Multimodal Representation Training Objective in PyTorch style}
\label{alg:clip}
\definecolor{codeblue}{rgb}{0.0,0.5,0.0}
\definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
\lstset{
  basicstyle=\fontsize{10pt}{9pt}\lstsansserif\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\color{codeblue},
  keywordstyle=\color{codekw},
}
\begin{lstlisting}[language=python]
# f: volume tokenizer (3D-CNN)
# F: pixel intensity filtering function
# ViT_seq: sequence model (transformer)
# ViT_st: study model (transformer)
# G: report encoder (gpt-2 transformer, pre-trained on reports by )
# E_sn: sequence name encoder (transformer)
# E_stn: study name encoder (LSTM)
# S: minibatch of N MRI Studies
# R: minibatch of matched N MRI Reports
# P_patdis: the patient discrimination projection layer
# lambda_patdis: patient discrimination loss weight
# tau, tau_p: temperature for clip and patient discrimination loss

def encode_sequence(sequence):
   # Encode the sequence name from the sequence metadata
   seq_name_encoded = E_sn(sequence.name) 
   # Tokenize series, concatenate name, forward pass f
   return  ViT_seq(torch.cat([f(F(sequence)),seq_name_encoded])) 

def encode_study(study):
   # Encode the study name from the study metadata
   study_name_encoded = E_st(study.name) 
   # Encode sequences, concatenate name, forward pass g
   encoded_seqs = torch.stack([encode_sequence(sequence) for sequence in study])
   return  ViT_st(torch.cat([encoded_seqs,study_name_encoded])) 

def patient_discrimination_loss(studies):
   # compute projected sequence embedding for patient discrimination loss
   seq_embs = []
   seq_maps = [] # maps each seq emb to the study it belongs to
   for i,study in enumerate(studies):
      seq_embs.extend([P_patdis(encode_sequence(sequence)) for sequence in study])
      seq_map.extend([i for sequence in study])
   seq_embs = torch.stack(seq_embs)
   # compute positive mask from seq_map
   seq_maps = torch.LongTensor(seq_maps)
   mask = (seq_maps[:,None] == seq_maps)
   masksum = mask.sum(dim=1)
   logits = torch.matmul(seq_embs,seq_embs.t())/tau_p
   logits.fill_diagonal_(-10)
   q = F.softmax(logits,dim=1)
   aggscores = (mask * q).sum(dim=1)
   return -torch.dot(aggscores.log(),1.0/masksum)
   
# Compute the MRI study and report features 
S_features = torch.stack([encode_study(study) for study in S])
R_features = G(R)
# Compute inner product between all MRI and Report features
logits = torch.matmul(S_features, R_features.t())*exp(tau)
# Targets: diagonal elements are the matching pairs
targets = torch.arange(logits.size(0))
# Cross-entropy loss for both mri-to-report and report-to-mri
loss_mri2report = F.cross_entropy(logits, targets)
loss_report2mri = F.cross_entropy(logits.t(), targets)
# Total loss is the average of both losses
loss_clip = (loss_mri2report + loss_report2mri) / 2
loss_patdis = patient_discrimination_loss(S)
loss = loss_clip + lambda_patdis * loss_patdis
\end{lstlisting}
\end{algorithm}
\end{minipage}
\vspace{-10pt}
\end{figure*}
% # Normalize the MRI and report features
% S_features = F.normalize(S_features, p=2, dim=1)
% R_features = F.normalize(R_features, p=2, dim=1)

